On Variants of Facility Location Problem with Outliers

In this work, we study the extension of two variants of the facility location problem (FL) to make them robust towards a few distantly located clients. First, $k$-facility location problem ($k$FL), a common generalization of FL and $k$ median problems, is a well studied problem in literature. In the second variant, lower bounded facility location (LBFL), we are given a bound on the minimum number of clients that an opened facility must serve. Lower bounds are required in many applications like profitability in commerce and load balancing in transportation problem. In both the cases, the cost of the solution may be increased grossly by a few distantly located clients, called the outliers. Thus, in this work, we extend $k$FL and LBFL to make them robust towards the outliers. For $k$FL with outliers ($k$FLO) we present the first (constant) factor approximation violating the cardinality requirement by +1. As a by-product, we also obtain the first approximation for FLO based on LP-rounding. For LBFLO, we present a tri-criteria solution with a trade-off between the violations in lower bounds and the number of outliers. With a violation of $1/2$ in lower bounds, we get a violation of $2$ in outliers.

==> High_Level_Idea_old_version.tex <==
\subsection{High Level Idea}
Let $I$ be an input instance of the LBUBFL problem. We work in the following steps:

\begin{enumerate}
    \item We first compute a tri-criteria solution $S^t$ to $I$. $S^t$ violates the lower bound by a factor of  $1/2$ denoted by $\alpha$ and the upper bound by a factor of $2$ denoted by $\beta$. $Cost(S^t) \le a_1 Cost(O)$ where $O$ is $Opt(I)$.
    
   \item We transform the instance $I$ into another instance $I_1$ of LBUBFL using the tri-criteria solution $S^t$. We show that $Cost(O_1) \le b Cost(S^t) + c Cost(O) \le  a_2 Cost(O)$ where $a_2 = b a_1 + c$.
    
    \item We transform the instance $I$ into an instance $I_2$ of LBFL, ignoring the upper bounds, using the tri-criteria solution $S^t$. We show that $Cost(O_2) \le b Cost(S^t) + c Cost(O) \le  a_2 Cost(O)$ where $a_2 = b a_1 + c$.
    
    
 %   \item We then create an instance $I_{cap}$ of CFLP ignoring the UBs. We show that $Cost(O_{cap}) \le d Cost(O_1) \le a_3 Cost(O)$ where $a_3 = d a_2$.
 
 \item We then create an instance $I_{cap}$ of CFLP from $I_2$. We show that $Cost(O_{cap}) \le d Cost(O_2) \le a_3 Cost(O)$ where $a_3 = d a_2$.
    
    \item We obtain an $\alpha$ approximate solution 
    $ AS_{cap}$ for $I_{cap}$ with $\beta$ violation in capacities. (for the time being we may assume $\beta = 2$. We will have to see the impact of capacity violation: in the discussion yesterday we assumed no capacity violation in AScap( lets say by using local search algo for CFLP) ). That is $Cost(AS_{cap}) \le \alpha Cost(O_{cap}) \le a_4 Cost(O)$ where $a_4 = a_3 \alpha$.
    
  %  \item From $ AS_{cap}$, we obtain a solution $S_1$ for $I_1$ such that cost of $ Cost(S_1) \le \alpha' Cost(AS_{cap}) \le a_5 Cost(O)$ where $a_5 = a_4 \alpha'$.
    
     \item From $ AS_{cap}$, we obtain a solution $S_2$ for $I_2$ such that cost of $ Cost(S_2) \le \alpha' Cost(AS_{cap}) \le a_5 Cost(O)$ where $a_5 = a_4 \alpha'$.....most probably we will construct solution to I directly from AScap.
     
  %  \item From $ S_1$, we obtain a solution $S$ for $I$ such that cost of $ Cost(S) \le  Cost(S_1) + Cost(O) \le (a_5 + 1) Cost(O)$.
  
   \item From $ S_2$, we obtain a solution $S$ for $I$ such that cost of $ Cost(S) \le  Cost(S_2) + Cost(O) \le (a_5 + 1) Cost(O)$.
    
\end{enumerate}


==> Intro_copy.tex <==
\section{Introduction}
Consider the problem of opening a given number of stores in a city where opening each store has an associated opening cost. Our aim is to open these stores such that the cost of opening the stores plus the cost servicing all the customers in the city from the nearest opened store is minimised. Such problems are called {\em facility location problems} where stores are the facilities and customers are the clients. In the above scenario, a few distant customers/clients can increase the cost of our solution disproportionately; such clients are called {\em outliers}. In this paper we first study facility location problem with outliers (FLO).
FLO and its variants were first introduced by Charikar \etal~\cite{charikar2001algorithms}. They also presented constant factor approximations for them.
%In this paper, we study a variant of facility location problem with outliers called {\em $k$-facility location problem with outliers} ($k$FLO). 
Formally, in FLO, we are given a set $\facilityset$ of $n$ facilities, a set $\cliset$ of $m$ clients and an integer $t$. Each facility $i \in \facilityset$ has an opening cost $f_i$ and cost of servicing a client $j \in \cliset$ from a facility $i \in \facilityset$ is $c(i,j)$ (we assume that the service costs are metric). We are allowed to leave bounded number ($t$) of clients unserved. The goal is to open a subset $\facilityset' \subseteq \facilityset$ of facilities such that the cost of opening the facilities and servicing $m-t$ clients from these opened facilities is minimised. 

In another variant of the problem, we are required to serve some minimum number of clients from an opened facility. Such a requirement arises naturally to ensure profitability in commerce and balancing loads in applications like transportation.
%In real life scenario, the stores have a minimum \textcolor{red}{sale} requirement to keep a check on profitability, that is, every store must serve some minimum number of clients to remain profitable. 
This minimum requirement is captured as lower bounds in facility location problems. Thus, in lower bounded FLPO (LBFLO), we are also given a lower bound $\lb{i}$ on the minimum number of clients that an opened facility must serve. \textcolor{red}{
The goal remains the same, to minimize the total cost...will see }
Since FLP is well known to be NP-hard, NP-hardness of FLO  and LBFLO follows.
We first present the first (constant factor) approximation for FLO using LP rounding techniques. Previous work \cite{charikar2001algorithms,FriggstadKR19} on the problem uses primal-dual schema or local search techniques. The result is interesting as LP-rounding based algorithms are easy to integrate with other solutions. In particular we get the following:
 
\begin{theorem}
There is a polynomial time algorithm that approximates facility location problem with outliers within a constant factor($12$) of the optimal solution.
\end{theorem}

FLO is shown to have an unbounded integrality gap~\cite{charikar2001algorithms} with solution to the standard LP. We get around this difficulty by guessing the most expensive  facility opened in optimal solution. We also present two tri-criteria solutions for lower bounded FLO problem, as stated in Theorem~\ref{thm_LBkFLO1} and~\ref{thm_LBkFLO} where a tri-criteria solution is defined as follows:
 
 \begin{definition}
A tri-criteria solution for LBFLO is an $(\alpha, \beta, \gamma)$- approximation solution $S$ that violates lower bounds by a factor of $\alpha$ and outliers by a factor of $\beta$ with cost no more than $\gamma OPT$ where $OPT$ denotes the cost of an optimal solution of the problem, $\alpha<1$ and $\beta>1$.
\end{definition}

\begin{theorem}
\label{thm_LBkFLO1}
A polynomial time $(1/4,2,O(1))$-approximation can be obtained for LBFLO problem.
\end{theorem}

The result in Theorem~\ref{thm_LBkFLO1} is obtained using LP rounding techniques. Both $FLO$ and lower bounded facility location(LBFL) are known to have unbounded integrality gaps using standard LP. We present another tri-criteria solution where we have improved the violation in lower bounds using some combinatorial techniques. In particular we present the following: 

\begin{theorem}
\label{thm_LBkFLO}
A polynomial time $(\alpha,\frac{1}{1-\alpha}, (3+\epsilon)(\frac{1+\alpha}{1-\alpha}))$-approximation can be obtained for LBFLO problem  for a small $\epsilon>0$ and a constant $\alpha=(0,1)$.
\end{theorem}
Note that violation in outliers and the cost of solution can be made arbitrarily small by choosing $\alpha$ close to 0. Similarly, violation in lower bound can be chosen close to 1 at increased factor loss in outliers and cost. That is, the above theorem present a trade-off between violation in outliers(/cost) and lower bounds. For $\alpha=1/2$, we get $2$-factor violation in outliers at $(9+3\epsilon)$ factor loss in cost.
 
\textbf{Motivation for future work and additional results: (May be we can motivation for thm1 an thm3.. or we can shift these paragraphs after thm 1 and thm3 respectively.) }
$k$-facility location problem with outliers($k$FLO) is a problem closely related to FLO. In $k$FLO, we are also given a bound $k$ on the maximum number of facilities that can be opened i.e.  $|\facilityset'| \le k$. Note that the approximation algorithm for FLO by Charikar~\etal~\cite{charikar2001algorithms} using primal dual technique is not directly extendable to $k$FLP. It will require more techniques like langrangian multipliers. Whereas local search techniques has not been very successful with cardinality constraint and non-uniform facility opening costs. However,
using our techniques of FLO, we have a polynomial time algorithm that approximates $k$FLO using  at most $k+1$ facilities exhibiting the power of LP rounding techniques. We believe that using pre-processing and strengthened LP techniques of Krishnaswamy \etal~\cite{krishnaswamy-kMO}, we can get rid of this $+1$ violation in cardinality giving us first constant factor approximation for $k$FLO problem. This also implies a tri-criteria approximation for Lower bounded $k$FLO(LB$k$FLO) problem using our techniques of Theorem~\ref{thm_LBkFLO}.
 
In Theorem~\ref{thm_LBkFLO}, we can choose $\alpha$ to be slightly greater than $1/2$ maintaining violations in outliers close to $2$. This in particular is interesting because by improving the violations to greater than $1/2$, it might be possible to get rid of violations in lower bound in LBFLO using techniques of Shi Li~\cite{Li_NonUnifLBFL} for general LBFL. In Shi Li's approximation for general LBFL maintaing $\alpha>1/2$ is crucial to get rid of violations in lower bound.

%$k$FLO is a common generalisation of {\em facility location problem with outliers (FLO)} when $k=n$ and {\em $k$-Median with outliers ($k$MO)}, when the facility opening costs are all $0$.
%$k$MO has also been shown to have an unbounded integrality gap with standard LP by Charikar~\etal~\cite{charikar2001algorithms}. Krishnaswamy \etal~\cite{krishnaswamy-kMO} showed that the LP gap arises between {\em almost-integral} (solution with at most two fractionally opened facilities) and {\em fully-integral} (a solution where all the facilities are opened integrally) solution. Therefore any solution based purely on  rounding the solution to standard LP must either violate cardinality by at least $+1$ or violate the number of outliers.
\textbf{Our Techniques: }
For FLO, starting with an LP solution $\rho^* = <x^*, y^*>$, we first eliminate the $x^*_{ij}$ variables and work with an auxilliary linear programming (ALP) relaxation involving only $y_i$ variables. This is achieved by converting $\rho^*$ into a  {\em complete solution} in which either $x^*_{ij}=y^*_{i}$ or $x^*_{ij}=0$. Using the ALP we identify the set of clients that we are going to serve fully. ALP is solved using iterative rounding technique to give a pseudo-integral solution{\footnote{A solution is said to be pseudo integral if there are at most two fractional facilities}}. We open both the facilities at a loss of factor $2$ in the cost by guessing the maximum opening cost of a facility in the optimal. Though the problem is known to have an unbounded integrality gap~\cite{charikar2001algorithms}, we get around it by guessing the cost of the most expensive facility opened by the optimal solution. The same technique gives us a constant factor approximation for $k$FLO problem using at most $k+1$ facilities. 
    
For LBFLO, we construct an instance $I'$ of FLO by ignoring the lower bounds and defining new facility opening cost for each $i \in \facilityset$. Then we solve FLO to get an approximate solution $AS'$. Every facility $i$ opened in solution $AS'$ might not serve $\geq \alpha\lb{i}$ clients because we ignored the lower bounds in $I'$. Therefore, we do some reassignments of clients served by these facilities (making some of them outliers) such that the cost of reassignment of clients served by a facility is same as the facility opening cost of the respective facility. We then close these facilities. The violation in outliers is at most $\frac{1}{1-\alpha}$ in the process.



\textbf{Related Work:} The facility location problem(FL) is a fundamental and well studied~\cite{Shmoys,ChudakS03,Jain:2001,Byrka07,Chudak98,Li13} problem in operational research and theoretical computer science. Lower bounds in FL were introduced by Karger and Minkoff \cite{Minkoff_LBFL} and Guha \etal~\cite{Guha_LBFL}. They independently gave constant factor approximations with constant factor violation in lower bounds whereas the first true constant factor($448$) for LBFL was given by Zoya Svitkina \cite{Zoya_LBFL} for uniform lower bounds. The factor was improved to $82.6$ by Ahmadian and Swamy \cite{Ahmadian_LBFL}. Later, for general LBFL, Shi Li~\cite{Li_NonUnifLBFL} presented a $4000$-factor approximation. Han \etal~\cite{Han_LBknapsackM} presented constant(380) factor approximation for lower bounded $k$-Median problem.
Han \etal~\cite{Han_LBkM} studied the general lower bounded $k$-facility location problem (LB$k$FL) to give a bi-criteria solution, that is, a constant factor approximation with constant factor violation in lower bounds. 


The problems of facility location and $k$-median with outliers were first defined by Charikar \etal~\cite{charikar2001algorithms} in the theory world. For FLO, they gave a $(3+\epsilon)$-approximation using primal dual technique. For a special case of the problem with uniform facility opening costs and doubling metrics Friggstad \etal~\cite{FriggstadKR19}
gave a PTAS using multiswap local search.

 $k$MO was also shown to have unbounded integrality gap by~\cite{charikar2001algorithms} and they gave a $4(1+1/\epsilon)$-approximation with $(1+\epsilon)$-factor violation in outliers. The factor was reduced to $(3+\epsilon)$ using local search technique by Friggstad \etal~\cite{FriggstadKR19} with same $(1+\epsilon)$-factor violation in outliers. Using a combination of local search and primal dual Chen ~\cite{chen-kMO} gave the first true constant factor approximation for the problem. Their approximation factor was large and was improved to $(7.081+\epsilon)$ by  Krishnaswamy \etal~\cite{krishnaswamy-kMO}. They uses strengthened linear program and iterative rounding techniques and theirs is the current best result for the problem.
 
 The only work that deals with lower bound and outliers together is by Ahmadian and Swamy~\cite{ahmadian_lboutliers}. They have given constant factor approximation for lower-bounded min-sum-of-radii with outliers and lower-bounded k-supplier with outliers problems using primal-dual technique. 
 
To the best of our knowledge, no results are known for LBFLO problem in the literature. The results known for FLO problem uses primal-dual/local search technique. %Infact, no result is known for lower bounded facility location problem with outliers(LBFLO) and lower bounded $k$-Median problem with outliers(LB$k$MO) as well.} %In this paper we first present a $12$-factor approximation for $k$FLO problem using the ideas of Krishnaswamy \etal~\cite{krishnaswamy-kMO}.}

\textbf{Organisation of the paper:} A constant factor approximation for FLO problem is given in Section~\ref{kFLPO} using LP roudning techniques. In Section~\ref{tri-criteria1} and~\ref{LBkFLO}, the tri-criteria approximations for LBFLO are presented. Finally we conclude with future scope in Section~\ref{conclusion}.

==> Intro_copy2.tex <==
\section{Introduction}
Consider the problem of opening a given number of stores in a city where opening each store has an associated opening cost. Our aim is to open these stores such that the cost of opening the stores plus the cost servicing all the customers in the city from the nearest opened store is minimised. Such problems are called {\em facility location problems} where stores are the facilities and customers are the clients. In the above scenario, a few distant customers/clients can increase the cost of our solution disproportionately; such clients are called {\em outliers}. In this paper we study facility location problem with outliers (FLO)
 and its extension.
Outliers were first introduced by Charikar \etal~\cite{charikar2001algorithms}. They also presented constant factor approximations for FLO and its variants using primal-dual schema.
%In this paper, we study a variant of facility location problem with outliers called {\em $k$-facility location problem with outliers} ($k$FLO). 
Formally, in FLO, we are given a set $\facilityset$ of $n$ facilities, a set $\cliset$ of $m$ clients and an integer $t$. Each facility $i \in \facilityset$ has an opening cost $f_i$ and cost of servicing a client $j \in \cliset$ from a facility $i \in \facilityset$ is $c(i,j)$ (we assume that the service costs are metric). The goal is to open a subset $\facilityset' \subseteq \facilityset$ of facilities such that the cost of opening the facilities and servicing at least $m-t$ clients from these opened facilities is minimised. 

In another variant of the problem, we are required to serve some minimum number of clients from an opened facility. Such a requirement arises naturally to ensure profitability in commerce and balancing loads in applications like transportation.
%In real life scenario, the stores have a minimum \textcolor{red}{sale} requirement to keep a check on profitability, that is, every store must serve some minimum number of clients to remain profitable. 
This minimum requirement is captured as lower bounds in facility location problems. Thus, in lower bounded FLPO (LBFLO), we are also given a lower bound $\lb{i}$ on the minimum number of clients that an opened facility $i$ must serve. The cost function remains the same.

Since FLP is well known to be NP-hard, NP-hardness of FLO  and LBFLO follows.
We present the first (constant factor) approximation for the problem.  In particular, we present the following result:

\begin{theorem}
\label{thm_flo}
There is a polynomial time algorithm that approximates facility location problem with outliers within a constant factor($12$) of the optimal solution.
\end{theorem}

Our result is obtained using LP rounding techniques. Though
FLO is shown to have an unbounded integrality gap~\cite{charikar2001algorithms} with solution to the standard LP,  we get around this difficulty by guessing the most expensive  facility opened in optimal solution. Previous work  \cite{charikar2001algorithms,FriggstadKR19} on the problem uses primal-dual schema or local search techniques.Though our result is weaker than $(3+\epsilon)$-approximation of Charikar \etal~\cite{charikar2001algorithms} that uses similar techniques of guessing the most expensive facility along with primal-dual schema, our result is interesting as LP-rounding based algorithms are easy to integrate with other solutions. For example, in $k$-facility location problem with outliers($k$FLO), we are  given an additional bound $k$ on the maximum number of facilities that can be opened i.e.  $|\facilityset'| \le k$. The primal-dual
solution by Charikar~\etal~\cite{charikar2001algorithms}  is not trivial to extend to $k$FLPO as it requires techniques like langrangian multipliers to deal with cardinality. 
Local search techniques have not been very successful to deal with the cardinality constraint with general facility opening costs. On the other hand, our solution for FLO  directly provides a similar result for $k$FLO using  at most $k+1$ facilities exhibiting the power of LP rounding techniques.
\textcolor{red}{Here we may note that result of Charikar~\etal~\cite{charikar2001algorithms} for $k$ median with outliers also violate the outliers. Thus, we do not expect to get a solution by extending their solution for FLO to $k$FLO without violating the outliers.}

Using an approximation for FLO as a black box, we also present the first approximation for LBFLO. To the best of our knowledge, no result is known for LBFLO in literature. A tri-criteria solution is obtained for the problem as stated in Theorem~\ref{thm_LBkFLO} where tri-criteria solution is defined as follows:
 
 \begin{definition}
A tri-criteria solution for LBFLO is an $(\alpha, \beta, \gamma)$- approximation solution $S$ that violates lower bounds by a factor of $\alpha$ and outliers by a factor of $\beta$ with cost no more than $\gamma OPT$ where $OPT$ denotes the cost of an optimal solution of the problem, $\alpha<1$ and $\beta>1$.
\end{definition}

\begin{theorem}
\label{thm_LBkFLO}
A polynomial time $(\alpha,\frac{1}{1-\alpha}, \lambda(\frac{1+\alpha}{1-\alpha})$-approximation can be obtained for LBFLO problem where $\alpha=(0,1)$ is a constant and $\lambda$ is an approximation factor for the FLO problem.
\end{theorem}
%Combination of LP rounding and combinatorial techniques is used to get Theorem~\ref{thm_LBkFLO}. 
Theorem~\ref{thm_LBkFLO} presents a trade-off between violation in outliers and lower bounds. That is, violation in outliers can be made arbitrarily small by choosing $\alpha$ close to 0. Similarly, violation in lower bound can be chosen close to 1 at the cost of increased violation in outliers. \textcolor{blue}{Similar result can be obtained for LB$k$FLO with $+1$ violation in cardinality (the violation is coming from $k$FLO).}
%For example, approximation for $k$MO by Krishnaswamy~\etal~\cite{krishnaswamy-kMO} can be used in our algorithm to get a tri-criteria, $(\alpha,\frac{1}{1-\alpha}, \lambda(\frac{1+\alpha}{1-\alpha}))$, solution for LB$k$MO for $\alpha=(0,1)$ where $\lambda=(7.08+\epsilon)$ is approximation factor of $k$MO in~\cite{krishnaswamy-kMO}.
 

%$k$FLO is a common generalisation of {\em facility location problem with outliers (FLO)} when $k=n$ and {\em $k$-Median with outliers ($k$MO)}, when the facility opening costs are all $0$.
%$k$MO has also been shown to have an unbounded integrality gap with standard LP by Charikar~\etal~\cite{charikar2001algorithms}. Krishnaswamy \etal~\cite{krishnaswamy-kMO} showed that the LP gap arises between {\em almost-integral} (solution with at most two fractionally opened facilities) and {\em fully-integral} (a solution where all the facilities are opened integrally) solution. Therefore any solution based purely on  rounding the solution to standard LP must either violate cardinality by at least $+1$ or violate the number of outliers.
\textbf{Our Techniques: }
For FLO, starting with an LP solution $\rho^* = <x^*, y^*>$, we first eliminate the $x^*_{ij}$ variables and work with an auxilliary linear programming (ALP) relaxation involving only $y_i$ variables. This is achieved by converting $\rho^*$ into a  {\em complete solution} in which either $x^*_{ij}=y^*_{i}$ or $x^*_{ij}=0$. Using the ALP, we identify the set of facilities to open in our solution. ALP is solved using iterative rounding technique to give a pseudo-integral solution (a solution is said to be pseudo integral if there are at most two fractional facilities). We open both the facilities at a loss of factor $2$ in the cost by guessing the maximum opening cost of a facility in the optimal. Once we identify the set of facilities to open, we can greedily assign the first $m-t$ clients in the increasing order of distance from the nearest opened facility. Thus, in the rest of the paper, we only focus on identifying the set of facilities to open.
    
For LBFLO, we construct an instance $I'$ of FLO by ignoring the lower bounds and defining new facility opening cost for each $i \in \facilityset$. An approximate solution $AS'$ to $I'$ is obtained using any approximation algorithm for FLO. Facilities serving less than $\alpha\lb{i}$ clients are closed and their clients are either reassigned to the other opened facilities or are made outliers. This leads to violation in outliers that is bounded by $\frac{1}{1-\alpha}$. Facility opening costs in $I'$ are defined to capture the cost of reassignments.


\textbf{Related Work:} %The facility location problem(FL) is a fundamental and well studied~\cite{Shmoys,ChudakS03,Jain:2001,Byrka07,Chudak98,Li13} problem in operational research and theoretical computer science. 
The problems of facility location and $k$-median with outliers were first defined by Charikar~\etal~\cite{charikar2001algorithms}.
Both the problems were shown to have unbounded integrality gap~\cite{charikar2001algorithms} with their standard LPs.
%Though FLO was shown to have unbounded integrality gap~\cite{charikar2001algorithms} using standard LP.
For FLO, they gave a $(3+\epsilon)$-approximation using primal dual technique by guessing the most expensive facility opened by the optimal solution. 
For a special case of the problem with uniform facility opening costs and doubling metrics, Friggstad~\etal~\cite{FriggstadKR19}
gave a PTAS using multiswap local search. %$k$-Median with outliers was also shown to have unbounded integrality gap using standard LP by Charikar~\etal~\cite{charikar2001algorithms} and 
For $k$MO, Charikar~\etal~\cite{charikar2001algorithms} gave a $4(1+1/\epsilon)$-approximation with $(1+\epsilon)$-factor violation in outliers. Using local search techniques, Friggstad~\etal~\cite{FriggstadKR19} gave $(3+\epsilon)$ and $(1+\epsilon)$-approximations with ($1+\epsilon$) violation in cardinality for general and doubling metric respectively. Chen~\cite{chen-kMO} gave the first true constant factor approximation for the problem using a combination of local search and primal dual. Their approximation factor is large and it was improved to $(7.081+\epsilon)$ by  Krishnaswamy~\etal~\cite{krishnaswamy-kMO} by strengthening the LP. They use iterative rounding framework and, their factor is the current best result for the problem.

 
 Lower bounds in FL were introduced by Karger and Minkoff~\cite{Minkoff_LBFL} and Guha~\etal~\cite{Guha_LBFL}. They independently gave constant factor approximations with violation in lower bounds. The first true constant factor($448$) approximation was given by Zoya Svitkina~\cite{Zoya_LBFL} for uniform lower bounds. The factor was improved to $82.6$ by Ahmadian and Swamy \cite{Ahmadian_LBFL}.  Shi Li~\cite{Li_NonUnifLBFL} gave the first constant factor approximation for general lower bounds, with the constant being large ($4000$). 
Han~\etal~\cite{Han_LBkM} studied the general lower bounded $k$-facility location  (LB$k$FL) 
violating the lower bounds.
%\st{to give a bi-criteria solution, that is, a constant factor approximation with constant factor violation in lower bounds. }
 Same authors~\cite{Han_LBknapsackM} removed the violation in the lower bound for the $k$-Median problem.
 
 The only work that deals with lower bound and outliers together is by Ahmadian and Swamy~\cite{ahmadian_lboutliers}. They have given constant factor approximation for lower-bounded min-sum-of-radii with outliers and lower-bounded k-supplier with outliers problems using primal-dual technique.
 
%}
%Infact, no result is known for lower bounded facility location problem with outliers(LBFLO) and lower bounded $k$-Median problem with outliers(LB$k$MO) as well.} %In this paper we first present a $12$-factor approximation for $k$FLO problem using the ideas of Krishnaswamy \etal~\cite{krishnaswamy-kMO}.}

\textbf{Organisation of the paper:} A constant factor approximation for FLO  is given in Section~\ref{kFLPO} opening using LP rounding techniques. In Section~\ref{LBkFLO}, the tri-criteria solution for LBFLO is presented. Finally we conclude with future scope in Section~\ref{conclusion}.

==> Intro_rd.tex <==
\section{Introduction}
Facility location problem (FL) is a well motivated and extensively studied problem. Given a set of facilities with facility opening costs and a set of clients with a metric specifying the connection costs between facilities and clients, the goal is to select a subset of facilities such that the total cost of opening the selected facilities and connecting clients to the opened facilities is minimized. 

With growing emphasis on e-commerce marketplace platforms where we have a central platform mediating between the seller and the buyer, it becomes important to keep a check on the availability and profitability of the central store. A store serving too less clients can be non-profitable and a store getting too many orders can lead to bad service to the customers. This scenario leads to what we call as the lower- and upper- bounded facility location (LBUBFL) problem.
%\textcolor{blue}{
There are several other applications requiring both the lower as well as the upper bound on the number of clients assigned to the selected facilities. In a real world transportation problem presented by Lim et al. in~\cite{Lim_transportation}, there are a set of carriers and a set of customers who wish to ship a certain number of cargoes through these carriers. There is a transportation cost associated to ship a cargo through a particular carrier. The goal of the company is to ship cargoes in these carriers such that the total transportation cost is minimized. There is a natural upper bound on the number of cargoes a carrier can carry imposed by the capacity of the carrier.  In addition, the shipping companies are required to engage their carriers with a \textquotedblleft minimum quantity commitment\textquotedblright when shipping cargoes to United States. 
Another scenario in which the problem can be useful is in the applications requiring balancing of load 
on the facilities along with maintaining capacity constraints.

In this paper, we study the facility location problem with lower and upper bounds where we are given a set of $C$ of clients and a set $F$ of facilities with lower bounds $B$ and upper bounds $U$. Setting up a facility at location $i$ incurs cost $f_i$(called the {\em facility opening cost}) and servicing a client $j$ by a facility $i$ incurs cost $\dist{i}{j}$ (called the {\em service cost}). We assume that the costs are metric, i.e., they satisfy the triangle inequality. Our goal is to open a subset $F' \subseteq F$ and serve the clients from the opened facilities such that every facility satisfies the lower and upper bound and the total cost of setting up the facilities and servicing the clients is minimised. The problem is known to be NP-Hard and we present a constant factor approximation violating the upper bounds by a factor of $3$ when both the lower and the upper bounds are uniform. %\textcolor{red}{The restricted variants of the problem with only the upper bounds or only the lower bounds are also known to be NP-hard~\cite{Minkoff_LBFL,Guha_LBFL}}.


Constant factor approximations are known for the problem with upper bounds only (popularly known as Capacitated Facility Location (CFL)) with~\cite{Shmoys,capkmByrkaFRS2013,GroverGKP18} and without violating the capacities using local search ~\cite{KPR,ChudakW99,mathp,paltree,mahdian_universal,zhangchenye,Bansal}/ LP rounding techniques~\cite{Anfocs2014}. Constant factor approximations are also known for the problem with lower bounds only with~\cite{Minkoff_LBFL,Guha_LBFL,Han_LBkM} and without violating the lower bounds~\cite{Zoya_LBFL,Ahmadian_LBFL,Li_NonUnifLBFL}. The only work that deals with the bounds on both the sides is due to Friggstad et al. \cite{friggstad_et_al_LBUFL},
%To the best of our knowledge, the only known result for the problem is by friggstad et al. \cite{friggstad_et_al_LBUFL}, they have considered
which deals with the problem with non-uniform lower bounds and uniform upper bounds.  They gave a constant factor approximation for the problem using LP-rounding,  violating both the upper and the lower bound by a constant factor. The technique cannot be used to get rid of the violation in the lower bounds even if they are uniform as the authors show an unbounded integrality gap for the problem.
%LP for the problem has been shown to have unbounded integrality gap in the same paper. %\textcolor{red}{The technique cannot be used to get rid of the violation in the lower bound even if we assume the lower bounds to be uniform because they use natural LP of the problem to bound the cost of the solution which is known to have unbounded integrality gap even for uniform lower bounds~\cite{friggstad_et_al_LBUFL}. Therefore, bi-criteria approximation is unaviodable if we use the LP}.
%Theorem~\ref{main_theo} summarises our result.



%\begin{theorem}
%\label{main_theo}
%There is a polynomial time algorithm that approximates lower- and upper- bounded facility location problem within a constant factor violating the capacities by a factor at most 3.
%\end{theorem}

\subsection{Related Work}
For capacitated facility location with  uniform capacities, Shmoys et al.~\cite{Shmoys} gave the first constant factor($7$) algorithm with a capacity blow-up of $7/2$.   An $O(1/\epsilon^2)$ factor approximation, with $(2 + \epsilon)$ violation in capacities, follows as a special case of C$k$FLP by Byrka et al.~\cite{capkmByrkaFRS2013}. Grover et al. \cite{GroverGKP18} reduced the capacity violation to $(1 + \epsilon)$
 using LP rounding techniques. For non-uniform capacities, An et al.~\cite{Anfocs2014} gave the first LP-based constant factor approximation algorithm without violating the capacities, by strengthening the natural LP. The local search technique has been particularly useful to deal with capacities. Korupolu et al.~\cite{KPR} gave the first constant factor ($8+\epsilon$) approximation for  uniform capacities, which was further improved by Chudak and Williamson  \cite{ChudakW99} to ($5.83+\epsilon$). The factor was subsequently reduced to $3$ by Aggarwal et al.~\cite{mathp}, which is also the best known result for the problem. For non-uniform capacities, Pal et al.~\cite{paltree} gave the first constant factor $(8.53 + \epsilon)$ approximation algorithm which was subsequently improved to $(7.88 +\epsilon)$ by Mahdian and Pal~\cite{mahdian_universal} and to  $(5.83+\epsilon)$ by Zhang et al.~\cite{zhangchenye} with the current best being $(5 + \epsilon)$ due to Bansal et al.~\cite{Bansal}.

Lower-Bounded Facility Location problem was introduced by Karger and Minkoff \cite{Minkoff_LBFL} and Guha et al. \cite{Guha_LBFL} independently in 2000. Both of them gave a bi-criteria algorithm, that is a constant-factor approximation with constant factor violation in lower bounds. Zoya Svitkina \cite{Zoya_LBFL} presented the first true constant factor($448$) approximation for the problem with uniform lower bounds by reducing the problem to CFL. This was later improved to $82.6$ by Ahmadian and Swamy \cite{Ahmadian_LBFL} using reduction to a special case of CFL called  Capacitated Discounted Facility Location. Later Shi Li \cite{Li_NonUnifLBFL} gave the first true constant ($4000$) factor approximation for the problem with non uniform lower bounds. He obtains his result by reducing the problem  to CFL via two intermediate problems called, LBFL-P(Lower bounded facility location with penalties) and TCSD(Transportation with configurable supplies and demands).
Han et al. \cite{Han_LBkM} gave a bi-criteria solution for the problem as a particular case of lower bounded $k$-FL problem when the lower bounds are non-uniform.

%\textcolor{red}{Another variant of LBFL, called Lower bounded $k$-Median problem(LB$k$M) was considered by Guo et al. \cite{Guo_LBkM} and Arutyunova and Schmidt \cite{arutyunova_LBkM} with uniform lower bounds, where they gave constant factor approximations for the problems by reducing them to CFL and LBFL respectively. For LB$k$FL problem with non-uniform lower bounds, Han et al. \cite{Han_LBkM} presented a bi-criteria algorithm giving $\alpha$ factor violaton in lower bounds and $\frac{1+\alpha}{1-\alpha}\rho$-approximation where $\rho$ is the approximation ratio for $k$FL problem and $\alpha$ is a constant. They also extend these results to LB$k$M and lower bounded knapsack median problem.}

Friggstad et al. \cite{friggstad_et_al_LBUFL} is the only work that deals with the problem with bounds on both the sides. The paper considers non-uniform lower bounds and uniform upper bounds. They gave a constant factor approximation, using LP rounding techniques, violating both the lower and the upper bounds. %$(\rho = max \{ \frac{(2\zeta+1)(2\eta+1)+\zeta}{\zeta} +4(\eta+1), \frac{2\eta}{\eta-1} \frac{\zeta+1}{\zeta}\})$ 
%for . They use LP rounding techniques to give violations in both upper and lower bounds.
%$\alpha= max\{\zeta, \frac{2\eta}{\eta-1}\}$  and $\beta = \frac{\zeta+1}{\zeta}$ violations in lower and upper bound respectively.

\subsection{High Level Idea}
Let $I$ be an input instance of the LBUBFL problem. We first present a tri-criteria solution violating both the lower as well as the upper bound and then extend the ideas of Zoya et al.~\cite{Zoya_LBFL}
to get rid of the violation in the lower bound.  Our tri-criteria solution is much simpler than that of Friggstad et al.~\cite{friggstad_et_al_LBUFL}. We reduce the problem instance $I$ to an instance $I_{cap}$ of CFL via a series of reductions ($I$ \rightarrow $I_1$ \rightarrow $I_2$ \rightarrow $I_{cap}$) in a  manner similar to Zoya et al.~\cite{Zoya_LBFL}. Also, facility trees are used to get rid of violation in the lower bounds in a similar manner.
%\cite{Zoya_LBFL} to get rid of the violations in the lower bound.
Capacities/upper bounds are violated at two places in \cite{Zoya_LBFL}: one while constructing a feasible solution for the $I_2$ instance; second while collecting at least $B$ clients at a facility in the facility trees. As the violation in $I_2$ cannot be handled, we defer the capacities to be handled later and ignore them while constructing $I_2$. We control the violation in the capacities while processing the facility trees by converting them into binary trees.
%We first compute a tri-criteria solution violating both the lower as well as the upper bound and then extend the ideas of Zoya et al.
%\cite{Zoya_LBFL} to get rid of the violations in the lower bound. Capacities are violated at two places in \cite{Zoya_LBFL}: one while constructing a feasible solution for the $I_2$ instance; second while collecting at least $B$ clients at a facility in the facility trees. As the violation in $I_2$ cannot be handled, we defer the capacities to be handled later and ignore them while constructing $I_2$. We control the violation in the capacities while processing the facility trees by converting them into binary trees.
Let $Cost(S)$ denotes the cost of a solution $S$. We work in the following steps:
\begin{enumerate}
    \item We first compute a tri-criteria solution $S^t$ to $I$ via clustering and filtering techniques. Let $\ell > 2$ be a fixed parameter, then $S^t$ violates the lower bound by a factor of  $(\ell-1)/\ell$ denoted by $\alpha$ and the upper bound by a factor of $2$ denoted by $\beta$. $Cost(S^t) \le O(\ell)Cost(O)$ where $O$ is an optimal solution to $I$.
    %$Opt(I)$.
    
   % To get rid of the violation in the lower bound, we reduce the problem to an instance  of CFL via a series of reductions. The key idea in the reduction is: let $n_i$ be the number of clients assigned to an open facility $i$ in $S^t$. If $i$ violates the lower bound, we create a demand of $B - n_i$ at $i$ in the CFL instance. The solution of the CFL instance then guides us to shut some of these open facilities and increase the assignments at others so as to respect the lower bound increasing the violation in the capacities by plus $1$. 
    
   \item We transform the instance $I$ into another instance $I_1$ of LBUBFL by moving the clients assigned to a facility $i$ by the  tri-criteria solution $S^t$ to $i$. The facilities opened by $S^t$ are assumed to be available free of cost. Let $O_1$ denote the optimal solution of $I_1$. A client $j$ is assigned to a facility $i$ if it was assigned to $i$ in $O_1$. The connection cost is bounded by the sum of the costs $j$ pays in $S^t$ and in $O_1$. Thus, $Cost(O_1) \le  Cost(S^t) + Cost(O) $.
   %$\le  (6\ell+ 7) Cost(O)$.
    
    \item The instance $I_1$ is transformed into another instance $I_2$ of LBFL, ignoring the upper bounds. The facility set is reduced to the facilities opened by $S^t$. If a client $j$ is assigned in $O_1$ to a facility $i$ not opened in $O_1$ then it is assigned to facility $i'$ nearest to $i$ and opened in $S^t$. The connection cost is bounded by twice the cost $j$ pays in $O_1$ by a simple triangle inequality. Let $O_2$ denote the optimal solution of $I_2$. Then,  $Cost(O_2) \le 2Cost(O_1)$.
    %$\leq 2 \cdot  (6\ell+7)Cost(O) = (12\ell+14)Cost(O)$ .
    
    \item Finally, we create an instance $I_{cap}$ of CFL from $I_2$. The key idea in the reduction is: let $n_i$ be the number of clients assigned to an open facility $i$ in $S^t$. If $i$ violates the lower bound, we create a demand of $B - n_i$ at $i$ in the CFL instance. The solution of the CFL instance then guides us to shut some of these open facilities and increase the assignments at others so as to respect the lower bounds. The process results in an increased violation in the capacities by plus $1$. Let $O_{cap}$ be an optimal solution of $I_{cap}$.  We show that $Cost(O_{cap}) \le (1+2\delta) Cost(O_2)$ for an appropriately chosen constant $\delta$.
    %$\le (1+2\delta)(12\ell+14)Cost(O)$.
    
    \item We obtain an 
    %$\alpha$ 
    approximate solution 
    $ AS_{cap}$ for $I_{cap}$.
    %with $\beta$ violation in capacities. (for the time being we may assume $\beta = 2$. We will have to see the impact of capacity violation: in the discussion yesterday we assumed no capacity violation in AScap
    (lets say by using local search algorithm~\cite{Bansal} for CFL). Thus, $Cost(AS_{cap}) \le (5 + \epsilon) Cost(O_{cap})$.
    %$ \le (5 + \epsilon) \cdot (1+2\delta) \cdot (12\ell+14) Cost(O)$.
    
     \item From $ AS_{cap}$, we obtain a solution $S_1$ for $I_1$ such that  capacities/upper bounds are violated by a factor of $(\beta + 1)$ with no violation in lower bounds and $Cost(S_1) \le (6\alpha/(2 \alpha - 1)) Cost(AS_{cap})$. Facility trees are constructed and processed bottom-up. Clients are moved up in the tree until we collect  at least $B$ clients at a facility. Whenever $B$ clients are assigned to a facility $i$, $i$ is opened and the tree rooted at $i$ is chopped off the tree and the process is repeated. To keep the violation in the upper bounds low, we create binary facility trees.
     
  
   \item From $ S_1$, we obtain a solution $S$ for $I$ by paying the facility cost and moving the clients back to their original location. Thus, $ Cost(S) \le  Cost(S^t) + Cost(S_1)$. 
   %$ \le (a_5 + 1) Cost(O)$.
    
\end{enumerate}

\subsection{Organisation of the Paper}
In Section \ref{tri-criteria}, we present a tri-criteria algorithm for LBUBFL using LP rounding techniques. In Section \ref{instI1} we reduce instance $I$ to $I_1$ and then $I_1$ to $I_2$, followed by reduction to  $I_{cap}$ in Section \ref{instIcap}. Then a bi-criteria algorithm for the problem is presented in Section \ref{bi-criteria}.

==> Introduction.tex <==
\section{Introduction}
Consider the problem of opening a given number of stores in a city where opening each store has an associated opening cost. Our aim is to open these stores such that the cost of opening the stores plus the cost servicing all the customers in the city from the nearest opened store is minimised. Such problems are called {\em facility location problems} where stores are the facilities and customers are the clients. In the above scenario, a few distant customers/clients can increase the cost of our solution disproportionately; such clients are called {\em outliers}. 
\textcolor{red}{The problem of facility location with outliers (FLO) and its variants were first introduced by Charikar \etal~\cite{charikar2001algorithms}. They also presented constant factor approximations for them.}
In this paper, we study a variant of facility location problem with outliers called {\em $k$-facility location problem with outliers} ($k$FLO). Formally, in FLO, we are given a set $\facilityset$ of $n$ facilities, a set $\cliset$ of $m$ clients, an integer $k$ and an integer $t$. Each facility $i \in \facilityset$ has an opening cost $f_i$ and cost of servicing a client $j \in \cliset$ from a facility $i \in \facilityset$ is $c(i,j)$ (we assume that the service costs are metric). We are allowed to leave bounded number ($t$) of clients unserved. The goal is to open a subset $\facilityset' \subseteq \facilityset$ of facilities such that the cost of opening the facilities and servicing $m-t$ clients from these opened facilities is minimised. In $k$FLO, we are also given a bound $k$ on the maximum number of facilities that can be opened i.e.  $|\facilityset'| \le k$. $k$FLO is a common generalisation of {\em facility location problem with outliers (FLO)} when $k=n$ and {\em $k$-Median with outliers ($k$MO)}, when the facility opening costs are all $0$.

In another variant of the problem, we are required to serve some minimum number of clients from an opened facility. Such a requirement arises naturally to ensure profitability in commerce and balancing loads in applications like transportation.
%In real life scenario, the stores have a minimum \textcolor{red}{sale} requirement to keep a check on profitability, that is, every store must serve some minimum number of clients to remain profitable. 
This minimum requirement is captured as lower bounds in facility location problems. Thus, in lower bounded FLPO (LBFLO), we are also given a lower bound $\lb{i}$ on the minimum number of clients that an opened facility must serve. \textcolor{red}{
The goal remains the same, to minimize the total cost...will see }
Since FLP is well known to be NP-hard, NP-hardness of $k$FLO  and LBFLO follows.
We present the first (constant factor) approximations for the problems.
%\textbf{Our Result:}  
In particular, we present the following results:
 
 \begin{theorem}
 There is a polynomial time algorithm that approximates $k$-facility location problem with outliers using  at most $k+1$ facilities, within a constant factor($12$) of the optimal solution.
 \end{theorem}
 
 
 \textcolor{cyan}{FLO is shown to have an unbounded integrality gap~\cite{charikar2001algorithms} with solution to the standard LP. We get around this difficulty by guessing the most expensive  facility opened in optimal solution. $k$MO has also been shown to have an unbounded integrality gap with standard LP by Charikar~\etal~\cite{charikar2001algorithms}. Krishnaswamy \etal~\cite{krishnaswamy-kMO} showed that the LP gap arises between {\em almost-integral} (solution with at most two fractionally opened facilities) and {\em fully-integral} (a solution where all the facilities are opened integrally) solution. Therefore any solution based purely on  rounding the solution to standard LP must either violate cardinality by at least $+1$ or violate the number of outliers.} 
 
 As a by product, we get the first constant factor approximation for FLO using LP rounding techniques. Previous work \cite{charikar2001algorithms,FriggstadKR19} on the problem uses primal-dual schema or local search techniques. The result is interesting as LP-rounding based algorithms are easy to integrate with other solutions in particular we get the following:
 
 \begin{corollary}
  There is a polynomial time algorithm that approximates facility location problem with outliers within a constant factor($12$) of the optimal solution.
 \end{corollary}
 
 We also present a tri-criteria solution for lower bounded FLO problem, as stated in Theorem~\ref{thm_LBkFLO} where a tri-criteria solution is defined as follows:
 
 \begin{definition}
A tri-criteria solution for LBFLO is an $(\alpha, \beta, \gamma)$- approximation solution $S$ that violates lower bounds by a factor of $\alpha$ and outliers by a factor of $\beta$ with cost no more than $\gamma OPT$ where $OPT$ denotes the cost of an optimal solution of the problem, $\alpha<1$ and $\beta>1$.
\end{definition}

\begin{theorem}
\label{thm_LBkFLO}
A polynomial time $(\alpha,\frac{1}{1-\alpha},12(\frac{1+\alpha}{1-\alpha}))$-approximation can be obtained for LBFLO problem where $\alpha=(0,1)$ is a constant.
\end{theorem}

Both $FLO$ and lower bounded facility location(LBFL) are known to have unbounded integrality gaps using standard LP. Therefore, the problem LBFLO also have unbounded integrality gap and any solution using LP rounding techniques to standard LP must violate both lower bounds and outliers.

\textbf{High Level Idea}
\begin{itemize}
    \item[1.] \textbf{$k$FLO:} Starting with an LP solution $\rho^* = <x^*, y^*>$, we first eliminate the $x^*_{ij}$ variables and work with an auxilliary linear programming (ALP) relaxation involving only $y_i$ variables. This is achieved by converting $\rho^*$ into a  {\em complete solution} in which either $x^*_{ij}=y^*_{i}$ or $x^*_{ij}=0$. Using the ALP we identify the set of clients that we are going to serve fully. ALP is solved using iterative rounding technique to give a pseudo-integral solution{\footnote{A solution is said to be pseudo integral if there are at most two fractional facilities}}. We open both the facilities at a loss of $+1$ in the cardinality constraint and a loss of factor $2$ in the cost by guessing the maximum opening cost of a facility in the optimal. The same technique gives us a constant factor approximation for FLO problem. Though the problem is known to have an unbounded integrality gap~\cite{charikar2001algorithms}, we get around it by guessing the cost of the most expensive facility opened by the optimal solution.
    
    \item[2.] \textbf{LBFLO:} We construct an instance $I'$ of $k$FLO by ignoring the lower bounds and defining new facility opening cost for each $i \in \facilityset$. Then we solve $k$FLO to get an approximate solution $AS'$. Every facility $i$ opened in solution $AS'$ might not serve $\geq \alpha\lb{i}$ clients because we ignored the lower bounds in $I'$. Therefore, we do some reassignments of clients served by these facilities(making some of them outliers) such that the cost of reassignment of clients served by a facility is same as the facility opening cost of the respective facility. We then close these facilities. The violation in outliers is at most $\frac{1}{1-\alpha}$ in the process. \textcolor{red}{Note that the techniques used in $FLO$ to get rid of violations in outliers can not be used here... because.. of lower bounds.. will have to see what to write }
\end{itemize}


\textbf{Related Work:} The facility location problem(FL) is a fundamental and well studied~\cite{Shmoys,ChudakS03,Jain:2001,Byrka07,Chudak98,Li13} problem in operational research and theoretical computer science. Lower bounds in FL were introduced by Karger and Minkoff \cite{Minkoff_LBFL} and Guha \etal~\cite{Guha_LBFL}. They independently gave constant factor approximations with constant factor violation in lower bounds whereas the first true constant factor($448$) for LBFL was given by Zoya Svitkina \cite{Zoya_LBFL} for uniform lower bounds. The factor was improved to $82.6$ by Ahmadian and Swamy \cite{Ahmadian_LBFL}. Later, for general LBFL, Shi Li~\cite{Li_NonUnifLBFL} presented a $4000$-factor approximation. Han \etal~\cite{Han_LBknapsackM} presented constant(380) factor approximation for lower bounded $k$-Median problem.
Han \etal~\cite{Han_LBkM} studied the general lower bounded $k$-facility location problem (LB$k$FL) to give a bi-criteria solution, that is, a constant factor approximation with constant factor violation in lower bounds. 


The problems of facility location and $k$-median with outliers were first defined by Charikar \etal~\cite{charikar2001algorithms} in the theory world. For FLO, they gave a $(3+\epsilon)$-approximation using primal dual technique. For a special case of the problem with uniform facility opening costs and doubling metrics Friggstad \etal~\cite{FriggstadKR19}
gave a PTAS using multiswap local search.

 $k$MO was also shown to have unbounded integrality gap by~\cite{charikar2001algorithms} and they gave a $4(1+1/\epsilon)$-approximation with $(1+\epsilon)$-factor violation in outliers. The factor was reduced to $(3+\epsilon)$ using local search technique by Friggstad \etal~\cite{FriggstadKR19} with same $(1+\epsilon)$-factor violation in outliers. Using a combination of local search and primal dual Chen ~\cite{chen-kMO} gave the first true constant factor approximation for the problem. Their approximation factor was large and was improved to $(7.081+\epsilon)$ by  Krishnaswamy \etal~\cite{krishnaswamy-kMO}. They uses strengthened linear program and iterative rounding techniques and theirs is the current best result for the problem.
 
 The only work that deals with lower bound and outliers together is by Ahmadian and Swamy~\cite{ahmadian_lboutliers}. They have given constant factor approximation for lower-bounded min-sum-of-radii with outliers and lower-bounded k-supplier with outliers problems using primal-dual technique. 
 
\textcolor{cyan}{To the best of our knowledge, no results are known for $k$FLO and LBFLO problems. The results known for FLO problem uses primal-dual/local search technique.} %Infact, no result is known for lower bounded facility location problem with outliers(LBFLO) and lower bounded $k$-Median problem with outliers(LB$k$MO) as well.} %In this paper we first present a $12$-factor approximation for $k$FLO problem using the ideas of Krishnaswamy \etal~\cite{krishnaswamy-kMO}.}

\textbf{Organisation of the paper:} A constant factor approximation for $k$FLO problem is given in Section~\ref{kFLPO}. In Section~\ref{LBkFLO}, the tri-criteria approximation for LBFLO is presented. Finally we conclude with future scope in Section~\ref{conclusion}.

==> LBFLO_rajni.tex <==

\section{Tri-Criteria for LB$k$FLO ($S^t$)}
Let $I=\{ C, F, c(i,j), f_i, B, k, t \}$ be the instance of LB$k$FLO. Let $O$ be the optimal solution of $I$. For each facility $i \in F$, let $N(i)$ be the set of closest $B$ clients of $i$. Next we construct an instance $I'$ of $k$FLO by dropping the lower bounds from $I$ and updating facility opening costs for each facility to be $f'_i = f_i + \lambda \sum_{j \in N(i)} c(i,j)$ where $\lambda$ is a constant that will be defined later.

\begin{lemma}
There is a solution to $I'$ of cost at most $F^*+ (\lambda+ 1) C^*$ where $F^*$ is the facility opening cost and $C^*$ is the connection cost in $O$.
\end{lemma}
\begin{proof}
{\em Feasibility:} Solution $O$ is a feasible solution to $I'$ because we have just dropped lower bounds in $I'$.

{\em Cost bound:} Connection cost is same as that of $O$. For facility opening cost, $\sum_{i \in O} f'_i= \sum_{i \in O}[ f_i + \lambda \sum_{j \in N(i)} c(i,j)] \leq F^* + \lambda C^*$.  Therefore, total cost is $ \leq F^* + \lambda C^* + C^* = F^*+ (\lambda+ 1) C^*$.
\end{proof}

Solve $I'$ using algorithm, in section 1, that gives $\delta$-approximation for $k$FLO without violating the outliers. Let the solution so obtained be $AS_{kFLO}$. 

\begin{equation}
    Cost(AS_{FLO}) \leq \delta Cost(I') \leq \delta (F^*+ (\lambda+ 1) C^*).
\end{equation}

\textcolor{blue}{Next we close facilities that are serving less than $\alpha B$ clients by either reassigning their clients to opened nearest neighbours or making their clients outliers. Consider all the facilities that are serving less than $\alpha B$ clients in $S'$. For each such facility $i$, let $N(o) \subseteq N(i)$ be the clients that are outliers. If $|N(o)| \geq \beta(1-\alpha)B$, make all the clients served by $i$ outliers otherwise reassign all the clients served by $i$ to a nearest facility $i' \neq i$ and close $i$. Let $S^t$ be the solution so obtained. Note that, all the facilities in $S^t$ serve at least $\alpha B$ clients.} \textcolor{red}{Note that we have only closed some facilities, so cardinality constraint will not be violated, that is, number of opened facilities are $\leq$ k}.

\begin{lemma}
Additional cost incurred in reassignment of clients for a facility $i$ is at most $f'_i$. We also incur $2$-factor loss in outliers.
\end{lemma}

\begin{proof}
Observe that if any facility $i$ serves less than $\alpha B$ clients than at least $(1-\alpha)B$ clients from set $N(i)$ are not assigned to $i$, that is, they were either outliers or were assigned to some other facility. 


\textcolor{red}{
\begin{itemize}
    \item If the number of outliers are $\ge \beta (1 - \alpha) B$, then we make all of them outliers at a violation of $\alpha / \beta (1 - \alpha)$ in outliers.
    \item otherwise the number of clients served from other facilities were at least $(1 - \beta)(1-\alpha)B$. We serve them from the nearest facility. Total cost is $\leq \frac{\alpha B}{(1 - \beta)(1-\alpha)B} \sum_{j \in N(i)} c(i,j) \leq f'_i$ for $\lambda =  .... $.....something like this...I don't know what do you want to say with $\lambda$ here.
\end{itemize}
we can set $\alpha$ and $\beta$ appropriately.}

%\begin{itemize}
  %  \item If number of outliers out of these $(1-\alpha)B$ clients are greater than $(1-\alpha)B/2$, then make all the clients outliers that were assigned to $i$ at 2 factor loss in outliers.
   % \item If number of outliers were less than $(1-\alpha)B/2$, then number of clients served from other facilities were at least $(1-\alpha)B/2$. Therefore, we can assign $\alpha B$ clients to nearest facility at $2$ factor loss in cost. Additional $2$ factor because of triangle inequality. Total cost is $\leq 4\frac{\alpha B}{(1-\alpha) B} \sum_{j \in N(i)} c(i,j) \leq f'_i$ for $\lambda = 4 \frac{\alpha B}{(1-\alpha) B} $
%\end{itemize}
%And the average distance of these $(1-\alpha)B$ clients from $i$ is at most $\sum_{j \in N(i)} c(i,j)/(1-\alpha)B$. Let $j'$ be one such client...\textcolor{red}{Might not exist.. all these $(1-\alpha)B$ clients can be outliers.}.. ok, will work for $t \leq B/4$.
\end{proof}

\begin{theorem}
We have a tri-criteria solution $S^t$ for instance $I$ with $\alpha > 1/2$ factor violation in lower bound, $\beta=2$ factor violation in outliers and $-$ factor loss in cost.
\end{theorem}

\begin{proof}

\end{proof}

\subsection{Instance $I_1$ of LB$k$FLO}
We transform the instance $I$ into another instance $I_1$ of LB$k$FLO by moving the clients assigned to a facility $i$ by the solution $S^t$ to $i$. The facilities opened by $S^t$ are assumed to be available free of cost. Note that outliers remains the same as in the solution $S^t$. Let $O_1$ denote the optimal solution of $I_1$. To construct a feasible solution $S_1$, we open a facility $i$ in $S_1$ iff it is opened in $O$. A client $j$ is assigned to a facility $i$ in $S_1$ if it was assigned to $i$ in $O$. If $j$ is an outlier in $O$, we make it an outlier. 
The cost $c( \sigma^t(j), \sigma^*(j))$ of serving $j$ from its new location is bounded as follows:
if $j$ is an outlier in $S^t$ and served by $O$ then by $ c(j, \sigma^*(j))$. If $j$ is served in both $O$ and $S^t$ then it is same as before.

\subsection{Instance $I_2$ of non-uniform LB$k$FLO}
The instance $I_1$ is transformed into another instance $I_2$. The facility set is reduced to the facilities opened by $S^t$ and some new facilities are added. For every client $j$ that was outlier in $S^t$, we make a dummy co-located facility with facility opening cost $0$ and lower bound $1$ (called special facilities). Note that there are two type of lower bounds, $B_i=1$ if $i$ is a $special$ facilities and $B_i=B$ otherwise. For feasible solution $S_2$: If a client $j$ was outlier in $O_1$, make it an outlier in $S_2$ and  if a client $j$ is assigned in $O_1$ to a facility not opened in $S^t$, then it is assigned to facility $i'$ nearest to $i$. \textcolor{blue}{Note that maximum number of facilities after adding special facilities is $k+t$, let $k'=k+t$ be the modified cardinality.} \textcolor{red}{ we can do this for $t \leq B/2$ because at least B/2 clients of $i \notin S^t$ were served by its nearest facility in $S^t$, so we can send these also at a loss of factor 2 in cost with no increase in outliers and lower bounds.. may be we can get rid of this restriction $B\leq t$ by making special facilities in $I_1$}.
 
 \subsection{CFL}
 Finally we create an instance $I_{cap}$ of CFL from $I_2$. Let $n_i$ be the number of clients assigned to an open facility $i$ in $S^t$. Recall that for a $special$ facility $n_i=0$. A facility is small if $0 < n_i \leq B$ and it is big otherwise. We create an instance of CFLP. Refer table \ref{tab:my_label} for the set of facilities, facility costs, capacities and demands. Let $F^t$ be the set of facilities so obtained. Note that the set of clients and the set of facilities are both $F^t$. 
 
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq B$ & $B$ & $B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > B$ & ($i_1$)$B$ & $0$& $\delta B l(i)$ \\
        & & ($i_2$) $n_i - B$ & $0$& $0$ \\
       
        % &  &
          \hline 
          {\em Special} & $n_i=0$ & $1$ & $B_i-1=0$ & M \\
          \hline
       % $3$ & $0$ & $B$ & $B$& $\delta B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 \begin{lemma}
 Cost of optimal solution to $I_{cap}$ is bounded.
 \end{lemma}
 
 \begin{proof}
 Feasible solution $S_{cap}$ to $I_{cap}$: Let $O_2$ be an optimal solution of $I_2$. As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $0 < n_i \le B$ (before taking more clients from outside) and it serves at least $B$ of its clients before sending out its clients to other (small) facilities otherwise. Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. \textcolor{red}{WLOG, we can also assume that the special facilities are always opened in $O_2$ as facility opening cost is $0$ in $I_2$ and these facilities serves the co-located clients, the clients that were outliers in $S^t$.}
 
 Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$ .
\begin{enumerate}
        \item If $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big. \textcolor{red}{Note that, $i$ can not be a $special$ facility.}
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
            \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. Thus, 
        $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = B = u_i$. %Thus capacities are respected.
      
         
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le B = u_{i_1}$.
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - B = u_{i_2}$.
         The second equality holds in each case as $i$ is closed in $O_2$.
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item Open free facility $i_2$ 
     %for $i_2 \in F_f$ (and 
     ($i$ is opened in $O_2$ \textcolor{red}{and $i$ is big..ng}) (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. 
\begin{enumerate}
    \item  If $i$ is big, we need not worry as $i_1$ and $i_2$ have no demand.
  \item  \textcolor{red}{ If $i$ is  special, we need not worry as $i$ has no demand.}
    \item Let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2) + \sum_{i' ~is ~special}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  +  \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)+ \sum_{i' ~is ~special}\rho^2(j_{i'}, i) = \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big}\rho^2(j_{i'}, i)+ \sum_{i' ~is ~special}\rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 
\end{enumerate}


Next, we bound the cost of the solution. The connection cost is same as that of $O_2$. %Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. \textcolor{red}{Note that $i$ can not be a special facility}. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities. The facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta n_i l(i)$.
\textcolor{red}{If $i$ is opened in $O_2$ and is $special$, then we have not opened it in our solution.}
\textcolor{blue}{Otherwise ( $i$ is opened in $O_2$ and is not $special$), $i$ must be serving at least $B$ clients and hence paying a cost of at least $B l(i)$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta B l(i)$.} Thus the facility cost is bounded by $2\delta Cost(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.
\end{proof}
 
 \section{Bi-criteria Solution $S_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$}
\label{bi-criteria}
Let $AS_{cap}$ be the approximation solution obtained for $I_{cap}$. 
\textcolor{red}{
Wlog, we may assume that no special facility is opened in $AS_{cap}$ ...not true...ok so it's true as $d_i \le u_i$ for all $i$ not special.}
Next we obtain a solution $S_1$ to $I_1$. Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand. $S_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $S_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, we define the assignments as follows:  For a big facility $i'$, assign all the clients co-located at $i'_1$ and $i'_2$ to $i$. For a small/special facility $i'$, assign the clients co-located at $i'$ to itself.  For small $i'$, additionally, we do the following  re-assignments (see Fig. \ref{type1}): $(i) $For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$.
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/Type 1 Assignments.jpg}
    \caption{($a$) $B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar F^t$.
    $(ii)$ $\sum_{i \ne i'} \rhobar^1(j_i, i') \le \beta U_{i'}$, $\forall$ $i' \in \bar F^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$.  
$\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$. Thus,
 %   
    %\item $\rhobar^1(j_{i'}, i') =$ original $n_{i'}$ clients $ %\rhobar^c(j_{i'}, i')$.....(1) $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$.....(2) Adding (1) and ((2) over all $i \ne i'$), we get
%
$\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{B, n_{i'}\} \le \beta U_{i'}$
\end{proof}

Note that $S_1$ so obtained may not still satisfy the lower bound requirement. In fact, 
 although each facility was assigned $n_i \ge  \alpha B \ge B/2$ clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  F^t$ be the set of facilities each of which is serving at least $B$ clients and  $\bar P =  F^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in F^t: \sum_{i}\rhobar^1(j_{i}, i') \ge B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ re-assignments.
 
 \begin{observation}
 If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
     Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha B \ge B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now try to group these facilities so that each group serves at least $B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in $\bar P$. For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $F^t$. Then, $G$ consists of edges $(i, \eta(i))$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair}, consisting of a pair of facilities say $i_i$ and  $i_2$ and denoted by $<i_{r_1}, i_{r_2}>$. Also, a facility $i$ from $P$, if present must be at the root of a tree. We try to process each tree bottom-up sending the clients of each facility to its parent. However doing so may result in too much violation in the capacities at the parent facility. 
 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{figures/tree.jpg}
    \caption{Binary tree conversion process: (a) Tree $\mathcal{T}$ of unbounded degree: $a<b<c<g,~c<d$. (b) Binary routing tree (intermediate stage). (c) Final tree.}
    \label{tree}
\end{figure}

 To keep the capacity violation in check, we convert each tree into a binary tree
 %\textcolor{red}{
 (see Fig. \ref{tree}): first of all, we treat the double-edge cycle, if any, as a single node for this purpose. Then, at every node $x$, arrange the children of $x$ from left to right in non-decreasing order of distance from $x$.
  For each child $y$ (except for the nearest child) of $x$, add an edge to its left sibling %with weight $2\dist{ y}{\eta(y)}$ 
  and remove the edge $( y, x)$. There is no change in the outgoing edge of the leftmost child of $x$. 
Let $\sigmaone(y)$ be the parent of  $y$ in the so constructed tree. Its easy to see that $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. Thus, we replace $\dist{y}{\sigmaone(y)}$ by $3 \dist{y}{\eta(y)}$ for all $y$. Henceforth, whenever we refer to distances, we mean the new edge weights. Now, every node has in-degree of at most $2$ with the in-degree of the root being at most $1$. 

Now we are ready to define our second type of re-assignments. Process the tree bottom-up as follows (see Fig. \ref{type2-3}): If $i$ has at least $B$ clients, open $i$ and disconnect $i$ from the tree by cutting the edge $(i, \sigmaone(i))$ else send its clients to its parent facility. The process is repeated till we reach the root. 



There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $<i_{r_1}, i_{r_2}>$. In the first case, we are done as $i$ is already open and has at least $B$ clients. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows (see Fig. \ref{type2-3}): ($i$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is at least $B$ then open the facility with more number of clients, say $i_{r_1}$ and send the clients of $i_{r_2}$ to $i_{r_1}$. %(in our case, we cannot have a scenario in which both have at least B clients. If $i_2$ is the facility at which the rest of the tree hangs then the number of clients at $i_1$ cannot be more than $B$.....this is not true in Zoya's case because there a tree hangs at both the ends of the double-edge loop which we have eliminated....Since the number of clients at $i_1$ is less than B..the number of clients along any edge is still less than B ....only for our understanding...to be deleted later)..
($ii$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is less than $B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$. i.e., $i$ is already open and has at least $B$ clients. Send the clients of $i_{r_1}$ and $i_{r_2}$ to $i$.
\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=40mm,scale=1.0]{figures/Type 2 Assignments.jpg}
		&& 
		\includegraphics[width=65mm,scale=1.0]{figures/Type 3 Assignments.jpg} 	
		\\
		\textbf{(A)}&&\ \ \textbf{(B)}& \ \
	\end{tabular}
	\caption{$B=4$ (A) Type 2 Assignments: (a) Before assignments. (b) After assignments.
	(B) Type 3 Assignments (i) Total clients at root pair $<i_{r_1},i_{r_2}>$ is at least $B$: (a) Before assignments. (b) After assignments: $i_{r_2}$ is open.  (ii) Total clients at root pair $<i_{r_1},i_{r_2}>$ is less than $B$: (a) Before assignments. (b) After assignments: $i_{r_1},i_{r_2}$ are both closed. 
	}
	\label{type2-3}
\end{figure}

%($i$) If both $i_1$ and $i_2$ have at least $B$ clients, open bot of them ($ii$) if one of them say $i_1$ has at least $B$ clients but $i_2$ doesn't then open $i_1$ and send the clients of $i_2$ to $i1$ ($iii$) If both of them have clients less than $B$ but in total they have at least $B$ clients, open any one of them, say $i_1$ and send the clients of the other to $i_1$
 
 
 We next bound the connection cost: the cost of first type of re-assignments is same as that of $AS_{cap}$.
 To bound the connection cost of second type, observe that we never send more than $B$ clients on any edge. 
 %In the second type of assignment, 
 Let a facility $i$ sends its (at most $B$ clients) to its parent. Since the facility $i$ was opened in $AS_{cap}$, it pays facility cost of $\delta l(i) min \{n_i, B\} \ge \delta l(i) \alpha B$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by $3 Cost_f(AS_{cap})/\alpha \delta$ where $Cost_f(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance. For the third type of re-assignments, the cost of sending (at most $B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ is not bounded by $B l(i)$. We bound the cost as follows: the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)B l(i)$. Hence the cost of type $3$ re-assignments is bounded by $3 Cost_c(AS_{cap})/ (2\alpha  - 1)$ where $Cost_c(.)$ is the connection cost of a solution to the $I_{cap}$ instance. Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1)$ for $\delta= (2\alpha-1)/6\alpha^2$.
 




==> LBUFL.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}
Let $F^t$ be the set of facilities opened by $S^t$. For a client $j$, let $\sigma^t(j)$ be the facility to which $j$ is assigned in $S^t$. For $i \in F$, let $n_i$ be the number of clients served by $i$ in $S^t$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i$ clients co-located with $i$. 
%For $i \in F^t$, $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin F^t$, $n_i = 0$.   
In $I_1$, our facility set is $F$ and the clients are at their new locations. 
$f^1_i = 0$ for $i \in F^t$ and $=f_i$ for $i \notin F^t$.
%We will show that there exists a feasible solution $S_1$ of $I_1$ such that $Cost(S_1)$ is bounded by $Cost(S^t) + Cost(O)$. 
For a client $j$, let $\sigma^*(j)$ be the facility serving $j$ in $O$.

\begin{lemma}
Cost of optimal solution of $I_1$ is bounded by $Cost(S^t) + Cost(O)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_1$ of $I_1$: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ iff it is assigned to $i$ in $O$. $S_1$ satisfies both the lower bound as well as the outliers as $O$ does so. 
\textcolor{red}{
The cost $c( \sigma^t(j), \sigma^*(j))$ of serving $j$ from its new location is bounded as follows:
if $j$ is an outlier in $S^t$ and served by $O$ then by $ c(j, \sigma^*(j))$ (see Fig. \ref{lemma1}).
if $j$ is an outlier in $O$ and served by $S^t$ then $j$ pays no cost in our solution as well. Else it is same as before.
}
Thus, the claim follows.


\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{figures/mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} \end{proof}


\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}


%section{Instance $I_2$} 
%\label{instI2}

  %For $i \in F$, let $n_i$ be the number of clients served by $i$ in $S^t$. Move these clients to $i$. Thus, there are $n_i$ clients co-located with $i$. For $i \in F^t$, $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin F^t$, $n_i = 0$. 
  %In $I_2$, our facility set is $F^t$ and the clients are at their new locations. 
  Next, we define an instance $I_2$ of LBFL, ignoring the outliers.
  Instance $I_2$ is same as $I_1$ without the upper bounds, except that the facility set is $F^t$ now. $f^2_i = 0$ for all $i \in F^t$. 
 % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.

\begin{lemma}
Cost of optimal solution of $I_2$ is bounded by $ 2Cost(O_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ of $I_2$: for $i$ \in $F^t$, open $i$ in $S_2$ if it is opened in $O_1$ and assign a client $j$ to it if it is assigned to $i$ in $O_1$. For $i$ \notin $F^t$, open its nearest facility $i'$ in $F^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $O_1$. $S_2$ satisfies the lower bound  as $O_1$ does so. However, it need not satisfy the upper bounds. The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $F^t$ to $i =  \sigma^1(j)$). Summing over all $j$'s we get the desired claim.

%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $F^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}




\section{Instance $I_{cap}$ for Capacitated Facility Location}
\label{instIcap}
For each facility $i \in F^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in F^t$, $i' \neq i$ and let $\delta$ be a constant chosen appropriately. We say that a facility $i$ is {\em small} if $0< n_i \leq B$ and it is {\em big} otherwise. Every big facility $i$ is split into two co-located facilities $i_1$ and $i_2$ . We split the set of clients, at $i$, also into two sets.  $B$ of these clients are placed at $i_1$ and the remaining $n_i - B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). The second type of big facilities are called {\em free}. 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{figures/mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$:
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $B = 4$ and it is $n_{i} - B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
%\textcolor{red}{ Let $F_f$ denote the set of free facilities (...will delete).} 
 Let $\bar F^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar F^t$. %In the $I_{cap}$ instance, we place demands  at all of these facilities. 
 The facility costs, capacities and demands are as shown in Table~\ref{tab:my_label} (also see Fig.~\ref{Mapping2}).
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq B$ & $B$ & $B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > B$ & ($i_1$)$B$ & $0$& $\delta B l(i)$ \\
        & & ($i_2$) $n_i - B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $B$ & $B$& $\delta B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.





\begin{lemma}
%A feasible solution $S_{cap}$ for 
Cost of optimal solution to 
$I_{cap}$ is bounded by
\textcolor{red}{
$(1+2\delta)Cost(S_2)$.
}
\end{lemma}

\begin{proof}
\textcolor{red}{
I think the proof should go through with $O_2$ replaced with $S^2$...remember $S^2$ is only existential...
}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost.
Let $O_2$ be an optimal solution of $I_2$. As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le B$ (before taking more clients from outside) and it serves at least $B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$ .
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{figures/O2_Scap assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
            \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. Thus, 
        $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = B = u_i$. %Thus capacities are respected.
      
         
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le B = u_{i_1}$.
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - B = u_{i_2}$.
         The second equality holds in each case as $i$ is closed in $O_2$.
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item Open free facility $i_2$ 
     %for $i_2 \in F_f$ (and 
     ($i$ is opened in $O_2$) (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
    Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)= \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big}\rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 


Next, we bound the cost of the solution. The connection cost is same as that of $O_2$. %Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities. The facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta n_i l(i)$.  If $i$ is opened in $O_2$, then it must be serving at least $B$ clients and hence paying a cost of at least $B l(i)$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta B l(i)$. Thus the facility cost is bounded by $2\delta Cost(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.
\end{proof}



\section{Bi-criteria Solution $S_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$}
\label{bi-criteria}


\textcolor{red}{
Here also I think everything should go through except that if there is a $j$ which was an outlier in $S^t$ is served by a facility $i$ in $AScap$, we don't know where to assign it back when constructing the solution $\bar S^2$ of $I_2$. We may have to drop such a client and make it an outlier which is understandable....and acceptable....Rest everything should work.
}
Next we obtain a solution $S_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 1)$ without violating the lower bound. 
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand. This is always feasible as $d_i \le u_i$. $S_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $S_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, we define the assignments as follows:  For a big facility $i'$, assign all the clients co-located at $i'_1$ and $i'_2$ to $i$. For a small facility $i'$, assign the clients co-located at $i'$ to itself.  For small $i'$, additionally, we do the following  re-assignments (see Fig. \ref{type1}): $(i) $For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$.
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/Type 1 Assignments.jpg}
    \caption{($a$) $B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar F^t$.
    $(ii)$ $\sum_{i \ne i'} \rhobar^1(j_i, i') \le \beta U_{i'}$, $\forall$ $i' \in \bar F^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$.  
$\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$. Thus,
 %   
    %\item $\rhobar^1(j_{i'}, i') =$ original $n_{i'}$ clients $ %\rhobar^c(j_{i'}, i')$.....(1) $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$.....(2) Adding (1) and ((2) over all $i \ne i'$), we get
%
$\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{B, n_{i'}\} \le \beta U_{i'}$
\end{proof}

Note that $S_1$ so obtained may not still satisfy the lower bound requirement. In fact, 
 although each facility was assigned $n_i \ge  \alpha B \ge B/2$ clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  F^t$ be the set of facilities each of which is serving at least $B$ clients and  $\bar P =  F^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in F^t: \sum_{i}\rhobar^1(j_{i}, i') \ge B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ re-assignments.
 
 \begin{observation}
 If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
     Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha B \ge B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now try to group these facilities so that each group serves at least $B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in $\bar P$. For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $F^t$. Then, $G$ consists of edges $(i, \eta(i))$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair}, consisting of a pair of facilities say $i_i$ and  $i_2$ and denoted by $<i_{r_1}, i_{r_2}>$. Also, a facility $i$ from $P$, if present must be at the root of a tree. We try to process each tree bottom-up sending the clients of each facility to its parent. However doing so may result in too much violation in the capacities at the parent facility. 
 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{figures/tree.jpg}
    \caption{Binary tree conversion process: (a) Tree $\mathcal{T}$ of unbounded degree: $a<b<c<g,~c<d$. (b) Binary routing tree (intermediate stage). (c) Final tree.}
    \label{tree}
\end{figure}

 To keep the capacity violation in check, we convert each tree into a binary tree
 %\textcolor{red}{
 (see Fig. \ref{tree}): first of all, we treat the double-edge cycle, if any, as a single node for this purpose. Then, at every node $x$, arrange the children of $x$ from left to right in non-decreasing order of distance from $x$.
  For each child $y$ (except for the nearest child) of $x$, add an edge to its left sibling %with weight $2\dist{ y}{\eta(y)}$ 
  and remove the edge $( y, x)$. There is no change in the outgoing edge of the leftmost child of $x$. 
Let $\sigmaone(y)$ be the parent of  $y$ in the so constructed tree. Its easy to see that $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. Thus, we replace $\dist{y}{\sigmaone(y)}$ by $3 \dist{y}{\eta(y)}$ for all $y$. Henceforth, whenever we refer to distances, we mean the new edge weights. Now, every node has in-degree of at most $2$ with the in-degree of the root being at most $1$. 

Now we are ready to define our second type of re-assignments. Process the tree bottom-up as follows (see Fig. \ref{type2-3}): If $i$ has at least $B$ clients, open $i$ and disconnect $i$ from the tree by cutting the edge $(i, \sigmaone(i))$ else send its clients to its parent facility. The process is repeated till we reach the root. 



There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $<i_{r_1}, i_{r_2}>$. In the first case, we are done as $i$ is already open and has at least $B$ clients. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows (see Fig. \ref{type2-3}): ($i$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is at least $B$ then open the facility with more number of clients, say $i_{r_1}$ and send the clients of $i_{r_2}$ to $i_{r_1}$. %(in our case, we cannot have a scenario in which both have at least B clients. If $i_2$ is the facility at which the rest of the tree hangs then the number of clients at $i_1$ cannot be more than $B$.....this is not true in Zoya's case because there a tree hangs at both the ends of the double-edge loop which we have eliminated....Since the number of clients at $i_1$ is less than B..the number of clients along any edge is still less than B ....only for our understanding...to be deleted later)..
($ii$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is less than $B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$. i.e., $i$ is already open and has at least $B$ clients. Send the clients of $i_{r_1}$ and $i_{r_2}$ to $i$.
\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=40mm,scale=1.0]{figures/Type 2 Assignments.jpg}
		&& 
		\includegraphics[width=65mm,scale=1.0]{figures/Type 3 Assignments.jpg} 	
		\\
		\textbf{(A)}&&\ \ \textbf{(B)}& \ \
	\end{tabular}
	\caption{$B=4$ (A) Type 2 Assignments: (a) Before assignments. (b) After assignments.
	(B) Type 3 Assignments (i) Total clients at root pair $<i_{r_1},i_{r_2}>$ is at least $B$: (a) Before assignments. (b) After assignments: $i_{r_2}$ is open.  (ii) Total clients at root pair $<i_{r_1},i_{r_2}>$ is less than $B$: (a) Before assignments. (b) After assignments: $i_{r_1},i_{r_2}$ are both closed. 
	}
	\label{type2-3}
\end{figure}

%($i$) If both $i_1$ and $i_2$ have at least $B$ clients, open bot of them ($ii$) if one of them say $i_1$ has at least $B$ clients but $i_2$ doesn't then open $i_1$ and send the clients of $i_2$ to $i1$ ($iii$) If both of them have clients less than $B$ but in total they have at least $B$ clients, open any one of them, say $i_1$ and send the clients of the other to $i_1$.
 
 
 Next we bound the capacity violation: Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta U$. Let $ i_c$ be the only child of the root (/root pair). Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect more than $2B$ clients at any node till we reach $i_c$. Now we have the following scenarios: Suppose $ i_c$ has less than $B$ clients, we have the following cases: ($i$)  the root node $i$ is in $P$ and it gets additional at most $B$ clients from $i_c$ making a total of at most $\pi_i + B \le \beta U + B \le (\beta + 1) U$ clients at $i$.
 ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at least $B$. Number of clients at $i_{r_1}$ and $i_{r_2}$ are at most $B$ and $2B$ respectively. Thus, the number of clients the opened facility gets is at most $3B \le 3 U$.
 ($iii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients less than $B$. Number of clients at the root pair and their nearest facility in $P$ are at most $B$ and $\beta U$ respectively. Thus, the number of clients the opened facility in $P$ gets is at most $\beta U + B \le (\beta + 1) U$. 
 %The case when $i_c$ has at least $B$ clients leads to the third scenario above and hence handled.
 
 We next bound the connection cost: the cost of first type of re-assignments is same as that of $AS_{cap}$.
 To bound the connection cost of second type, observe that we never send more than $B$ clients on any edge. 
 %In the second type of assignment, 
 Let a facility $i$ sends its (at most $B$ clients) to its parent. Since the facility $i$ was opened in $AS_{cap}$, it pays facility cost of $\delta l(i) min \{n_i, B\} \ge \delta l(i) \alpha B$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by $3 Cost_f(AS_{cap})/\alpha \delta$ where $Cost_f(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance. For the third type of re-assignments, the cost of sending (at most $B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ is not bounded by $B l(i)$. We bound the cost as follows: the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)B l(i)$. Hence the cost of type $3$ re-assignments is bounded by $3 Cost_c(AS_{cap})/ (2\alpha  - 1)$ where $Cost_c(.)$ is the connection cost of a solution to the $I_{cap}$ instance. Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1)$ for $\delta= (2\alpha-1)/6\alpha^2$.
 




==> Tri-criteria-I.tex <==
\section{A simple tri-criteria for LBFLO }
\label{tri-criteria1}
In this section we present a tri-criteria approximation for LBFLO problem with $1/4$-factor violation in lower bound and $2$-factor violation in outliers at a constant factor loss in cost. Following is the LP relaxation for LBFLO problem where for each $i \in \facilityset$, $y_i$ indicates if facility $i$ is opened, for each $i \in \facilityset$ and $j \in \cliset$, $x_{ij}$ indicates if client $j$ is assigned to facility $i$ and for each $j \in \cliset$, $z_j$ indicates if client $j$ is an outlier.

\label{{LBFLO}}
$\text{Minimize}~\mathcal{C}ostLBFLO(x,y,z) = \sum_{j \in \cliset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
\text{subject to} &\sum_{i \in \facilityset}{} x_{ij} + z_j \geq 1 & \forall ~\singleclient \in \clientset \label{LbkFLo_const1}\\ 
& \lb y_i \leq \sum_{j \in \cliset}x_{ij}  & \forall~ \singlefacility \in \facilityset \label{LbkFLo_const2}\\
%& \sum_{i \in \facilityset}y_{i} \leq k  \label{LbkFLo_const3}\\ 
& \sum_{j \in \clientset} z_{j} \leq t &  \label{LbkFLo_const4}\\   
&  x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LbkFLo_const5}\\ 
& y_i,x_{ij},z_j \in  [0,1]  \label{LPFLP_const5}
\end{eqnarray}

Constraints~\ref{LbkFLo_const1} ensure that every client is either served or is an outlier. Constraints~\ref{LbkFLo_const2} and~\ref{LbkFLo_const4} satisfies the lower bounds and number of outliers respectively. Constraints~\ref{LbkFLo_const5} are standard facility location constraint saying that a client is assigned to an open facility only. Let $opt=<x^*,y^*,z^*>$ be the optimal LP solution for the above LP.

A solution is said to be an {\em integral open solution} if all the facilities are either fully opened or fully closed, i.e, $y_i=[0,1]$ for all $i \in \facilityset$. Next we will construct an integral open solution $S=<\bar{x}, \bar{y}, \bar{z}>$. The solution $S$ is created in two steps: ($1$) First we create solution $S_{out}= <x', y', z'>$ by removing the clients that are outliers to a large extent($\geq 1/\lambda$) in $opt$ where $\lambda$ is a parameter to be fixed later, ($2$) Use clustering and rounding techniques to obtain an integral open solution for the remaining clients. Formally, in step 1, for all $j \in \cliset$ and $i \in \facilityset$, set $z'_{j}=1$ and $x'_{ij}=0$ if $z^*_{j} \geq 1/\lambda$. Otherwise, set $z'_{j}=0$ and $x'_{ij}=x^*_{ij}$. For all $i \in \facilityset$, $y'_{i}=y^*_{i}$. Note that in step 1 we just incur at most $\lambda$-factor in outliers. Also, $CostLBFLO(S_{out}) \leq CostLBFLO(opt)$. 

Next we will describe the Step 2 in detail. Let $\AVG{j}$ be the average connection cost for a client $j \in \cliset$ after Step 1, that is, $\AVG{j}=\sum_{i \in \facilityset} \dist{i}{j}x'_{ij}/\sum_{i \in \facilityset} x'_{ij}$. The clients are now considered in increasing order of radius $\lambda\AVG{j}$. Let $j$ be a client in this order, remove all the clients $k$ such that $c(j,k) \leq 2\lambda max \{ \AVG{j},\AVG{k} \}$ and repeat the process with the left over clients. Let $\clientset' \subset \cliset$ be the set of remaining clients after all the clients have been considered. Note that for any clients $j, k \in \clientset'$  the following property is satisfied: $c(j,k) > 2\lambda max \{ \AVG{j},\AVG{k} \}$. %The facility set $\facilityset$ is now partitioned into disjoint partitions $\cluster{j}$ by assigning each facility $i$ to the nearest client $j \in \clientset'$. Notice that if $\F{j}$ is the set of facilities within radius $\lambda\AVG{j}$, then $\F{j} \subseteq \cluster{j}$ for all $j \in \clientset'$. 
 The total extent up to which facilities are opened in $\F{j}$ after Step 1 is $\geq (1-1/\lambda)(\sum_{i \in \facilityset} x'_{ij}) \geq (1-1/\lambda) 1/\lambda$ where the last inequality follows because every client is served to an extent of at least $1/\lambda$ after first step. To obtain an integral open solution, for all $j \in \clientset'$, we open the cheapest(lowest facility opening cost) facility say $\iofj \in \F{j}$ and transfer all the assignments coming on to the facilities in $\cluster{j}$ to $\iofj$. Formally, set $\bar{y}_{\iofj}=1$, $\bar{x}_{\iofj j} = \sum_{i \in \cluster{j}}x'_{ij}$ and $\bar{y}_{i}=0$, $\bar{x}_{ij}=0$ for all $j \in \cliset$ and $i \neq \iofj$. Set $\bar{z}_{j} = z'_{j}$ for all $j \in \cliset$.

\begin{lemma}
The integral open solution $S=<\bar{x},\bar{y},\bar{z}>$ violates lower bound by $\alpha=1/4$ and outliers by $\gamma=2$ at constant(?) factor loss in cost.
\end{lemma}

\begin{proof}
   Set $\lambda=1/2$.
\end{proof}
   


==> conclusion.tex <==
\section{Conclusion}
\label{conclusion}
In this paper, we first presented a $12$-factor approximations for $k$-facility location problem with outliers using at most $k+1$ facilities. We round the LP solution using an iterative rounding algorithm to obtain an integral solution with $k+1$ opened facilities. Though the problem is known to have unbounded integrality gap using natural LP, our result shows that the gap arises between these solutions with $k+1$ and $k$ facilities. Next, we have given a tri-crtieria, $(\alpha, \frac{1}{1-\alpha}, 12\frac{1+\alpha}{1-\alpha})$ approximation for general LBFLO. Both FLO and LBFL problems are known to have unbounded integrality gap and therefore, violation in both are unavoidable using LP rounding techniques to standard LP.

We believe that our solution with $k+1$ facilities for $k$FLO can be converted to a solution with $k$ facilities using pre-processing and strengthened LP techniques of krishnaswamy \etal~\cite{krishnaswamy-kMO} giving the first true approximation for $k$FLO problem. This also extends our tri-criteria solution to lower bounded $k$-facility location problem with outliers (LB$k$FLO) and lower bounded $k$-Median problem with outliers.

 It will be interesting and challenging to get rid of violations in lower bounds in LBFLO using techniques of Shi Li~\cite{Li_NonUnifLBFL} for general LBFL. Knapsack Median and Matroid Median are two well known, closely related problems to $k$-facility location problem. Our results for $k$FLO can be modified to work for Knapsack Median with Outliers and Matroid Median with Outliers.
